FinanceBench: A New Benchmark for Financial Question Answering

FinanceBench is a first-of-its-kind test suite for evaluating the performance of LLMs on open book financial question answering (QA). It comprises 10,231 questions about publicly traded companies, with corresponding answers and evidence strings. The questions in FinanceBench are ecologically valid and cover a diverse set of scenarios. They are intended to be clear-cut and straightforward to answer to serve as a minimum performance standard. We test 16 state of the art model configurations (including GPT-4-Turbo, Llama2 and Claude2, with vector stores and long context prompts) on a sample of 150 cases from FinanceBench, and manually review their answers (n=2,400). The cases are available open-source. We show that existing LLMs have clear limitations for financial QA. Notably, GPT-4-Turbo used with a retrieval system incorrectly answered or refused to answer 81% of questions. While augmentation techniques such as using longer context window to feed in relevant evidence improve performance, they are unrealistic for enterprise settings due to increased latency and cannot support larger financial documents. We find that all models examined exhibit weaknesses, such as hallucinations, that limit their suitability for use by enterprises.

==> tables/table1.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage[normalem]{ulem}
% % \useunder{\uline}{\ul}{}
% \begin{table*}[htbp]
% \small
% \centering
% \begin{tabular}{l|cccccc|c}
% \hline\hline
% & \begin{tabular}[c]{@{}l@{}}Numerical reasoning:\\ multiple financial\\ statements\end{tabular} & \begin{tabular}[c]{@{}l@{}}Numerical reasoning:\\ single financial\\ statement\end{tabular} & \begin{tabular}[c]{@{}l@{}}Information\\ extraction\end{tabular} & \begin{tabular}[c]{@{}l@{}}Overall \%\\ correct\end{tabular} \\
% \hline\hline
% \begin{tabular}[c]{@{}l@{}}GPT4\\ No context\end{tabular} & 0\% & 3\% & 0\% & \textbf{1\%} \\
% \begin{tabular}[c]{@{}l@{}}GPT4\\ All docs in\\ one vector store\end{tabular} & 13\% & 21\% & 21\% & \textbf{18\%} \\
% \begin{tabular}[c]{@{}l@{}}GPT4\\ One doc per\\ vector store\end{tabular} & 13\% & 39\% & 29\% & \textbf{26\%} \\
% \begin{tabular}[c]{@{}l@{}}Llama2\\ One doc per\\ vector store\end{tabular} & 15\% & 12\% & 29\% & \textbf{18\%} \\
% \begin{tabular}[c]{@{}l@{}}GPT4\\ Evidence \\ strings\end{tabular} & \textbf{51\%} & \textbf{73\%} & \textbf{86\%} & \ul{\textbf{68\%}} \\
% \begin{tabular}[c]{@{}l@{}}Anthropic\\ Long\\ context\end{tabular} & 23\% & 42\% & 57\% & \textbf{39\%} \\
% \textbf{\begin{tabular}[c]{@{}l@{}}\% of\\ type\\ correct\end{tabular}} & \textbf{19\%} & \textbf{32\%} & \ul{\textbf{37\%}} & \\
% \hline\hline
% \end{tabular}
% \label{tab:metrics_performance}
% \end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% SECOND IMPLEMENTATION %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[htbp]
\small
\centering
\begin{tabular}{l|cccccc|c}

& \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}GPT4\\ No context\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}GPT4\\ All docs in\\ one vector store\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}GPT4\\ One doc per\\ vector store\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Llama2\\ One doc per\\ vector store\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}GPT4\\ Evidence \\ strings\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Anthropic\\ Long\\ context\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\% of\\ type\\ correct\end{tabular}} \\
\hline
\hline
\begin{tabular}[c]{@{}l@{}}Numerical reasoning:\\ multiple financial\\ statements\end{tabular} & 0\%                                                                           & 13\%                                                                                              & 13\%                                                                                          & 15\%                                                                                            & \textbf{51\%}                                                                          & 23\%                                                                                   & \textbf{19\%}                                                           \\
\hline
\begin{tabular}[c]{@{}l@{}}Numerical reasoning:\\ single financial\\ statement\end{tabular}    & 3\%                                                                           & 21\%                                                                                              & 39\%                                                                                          & 12\%                                                                                            & \textbf{73\%}                                                                          & 42\%                                                                                   & \textbf{32\%}                                                           \\
\hline
\begin{tabular}[c]{@{}l@{}}Information\\ extraction\end{tabular}                               & 0\%                                                                           & 21\%                                                                                              & 29\%                                                                                          & 29\%                                                                                            & \textbf{86\%}                                                                          & 57\%                                                                                   & {\ul \textbf{37\%}}                                                     \\
\hline
\textbf{\begin{tabular}[c]{@{}l@{}}Overall \%\\ correct\end{tabular}}                          & \textbf{1\%}                                                                  & \textbf{18\%}                                                                                     & \textbf{26\%}                                                                                 & \textbf{18\%}                                                                                   & {\ul \textbf{68\%}}                                                                    & \textbf{39\%}                                                                          &                                                                         \\ 
\end{tabular}
\caption{Model performance on the three types of metrics-generated questions}
\label{tab: metrics_performance}
\end{table*}

==> tables/table3.tex <==
\begin{table}[]
\begin{tabular}{l|cc|c}
\toprule
                      & \textbf{GPT-4}                                         & \textbf{Llama2}                                        & \textbf{Average}                                       \\
\midrule
\textbf{Correct}      & \begin{tabular}[c]{@{}c@{}}4,584\\ (45\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}3,595\\ (35\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}4,090\\ (40\%)\end{tabular} \\
\midrule
\textbf{Incorrect}    & \begin{tabular}[c]{@{}c@{}}976\\ (10\%)\end{tabular}   & \begin{tabular}[c]{@{}c@{}}6,156\\ (60\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}3,566\\ (35\%)\end{tabular} \\
\midrule
\textbf{Refusal}      & \begin{tabular}[c]{@{}c@{}}4,671\\ (46\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}480\\ (5\%)\end{tabular}    & \begin{tabular}[c]{@{}c@{}}2,576\\ (25\%)\end{tabular} \\
\midrule
\textbf{Failure rate} & 56\%                                                   & 65\%                                                   & 60\% \\
\bottomrule
\end{tabular}
\caption{Performance of two models on the full 10,231 entry dataset in \textsc{FinanceBench}, evaluated automatically.}
\label{tab:eval_performance}
\end{table}
